The variational structure of the space of holonomic measures

Roughly speaking, holonomic measures are parametric varifolds without boundary. They provide a setting appropriate for the analysis of many variational problems. In this paper, we characterize the space of variations for these objects, and we use the characterization to formulate stability conditions that are strictly more general than the Euler-Lagrange equations. We also use this characterization to deduce higher-dimensional analogues of energy conservation and weak KAM. Along the way, we characterize the distributions that arise as derivatives of families of Borel probability measures on smooth manifolds.

==> cobordisms.tex <==
Let $\mu\in\holonomic$ be a holonomic measure. Assume that there is a cycle $\alpha$, $\partial\alpha=0$, such that $\eta$ such that the measure $\mu_\alpha$ induced by it satisfies 
\[\supp\mu_\alpha\subseteq\supp\mu.\]
Then 

==> general_deformations.tex <==
In this section we will work on a smooth manifold $P$ that will later be taken to be $T^nM$.

Let $\mu_s$ be a family of Borel measures on the manifold $P$ parameterized by a real parameter $s$ with values in an open interval $J\subseteq\R$ that contains 0. We say that the family $\mu_s$ is \emph{differentiable} at 0 if there is a distribution $\eta\in\distributionsP$ such that, for every function $f\in C^\infty_c(P)$,
\[\left.\frac{d}{ds}\right|_{s=0}\int f\,d\mu_s=\langle\eta,f\rangle.\]
The distribution $\eta$ is the \emph{derivative} $d\mu_s/ds|_{s=0}$ of $\mu_s$ at 0.

\begin{rmk}
This is just one way to define differentiability of families of distributions; other ways have been explored for example in \cite{smolyanov}.
\end{rmk}

In this section we will investigate which measures can arise as derivatives of families of measures.



\begin{prop}
  For every measure $\mu$ and every distribution $\eta$, there exists a family of signed measures with 
  \[\mu_0=\mu\quad\textrm{and}\quad\left.\frac{d\mu_s}{ds}\right|_{s=0}=\eta.\]
\end{prop}
\begin{proof}
Take a mollifier $\psi$ and a tuple $F$ of generating vector fields. Then for example the family $\mu_s=\psi*_{sF}(\mu_0+s\eta)$ has the required properties.
\end{proof}

For families of \emph{positive} measures, the situation is different. 




\begin{thm}\label{thm:generalfamilies}
 Let $\mu$ be a positive measure and let $\eta$ be a distribution.
 Denote by $\posfuncs$ the space of nonnegative functions $f\in C^\infty_c(P)$ that vanish identically on $\supp \mu$.
 Then there exists a family $\mu_s$ of positive measures with derivative $d\mu_s/ds|_{s=0}=\eta$ and $\mu_0=\mu$ if, and only if, $\eta$ satisfies the following condition:
 \begin{equation}\label{eq:conditionD}\tag{\diffcondition}
  \textrm{$\langle\eta,f\rangle=0$ for every $f\in\posfuncs$. }
 \end{equation}
 If $\mu$ is a probability measure and $\langle\eta,1\rangle=0$, then $\mu_s$ is a family of probability measures too, when it exists.
\end{thm}

\begin{rmk}
 Condition \diffcondition\ implies that $\supp\eta\subseteq\supp\mu$.

 Appart from this, Condition \diffcondition\ is relevant only when $\supp\mu$ has parts that are very thin --- only one point thick. 
 
 For example, if $P=\R$, $\mu$ is the Dirac delta $\delta_0$, and $\rho:\R\to\R\in C^\infty_c(\R)$ is a cutoff function ($\rho\geq0$, $\rho\equiv 1$ in a neighborhood of 0 and $\rho\equiv 0$ outside a slightly larger neighborhood), then taking $f(x) = \rho(x)\sum_{i\geq2}c_i x^i$ (with $c_2$ large enough to ensure that $f\geq0$) we see that $\eta$ must be of the form $c_1\delta_0+c_2\partial\delta_0$, for involving any higher-degree derivatives would contradict the condition.
 
 On the other hand, if we again had $P=\R$, but now $\mu=\chi_{[0,1]}$ the characteristic function on the unit interval, then as long as $\supp\eta\subset\supp\mu$, $\eta$ can be any distribution and still comply with Condition \diffcondition.
\end{rmk}


 \begin{lem}\label{lem:variationpoint}
  Let $k>1$, and fix a point $p\in P$. Let $\eta_p$ be a distribution supported on $p$ that satisfies Condition \ref{eq:conditionD}.
 Then there is a family of positive measures $\mu_{s}^p$ such that $\mu_0^p=\mu$ and
 \[\left.\frac{d\mu_{s}^p}{ds}\right|_{s=0}=\eta_p.\]
 Moreover, the dependence of $\mu_s^p$ on $p$ is measurable.
 
  If $\mu$ is a probability measure and $\langle\eta_p,1\rangle=0$, then $\mu_s^p$ is a family of probability measures too, when it exists.
\end{lem}

For the proof of the lemma we will need a metric defined on the space of distributions involving up to $k^{\textrm{th}}$ derivatives and given by
\[\dist_k(\theta_1,\theta_2)=\sum_{j=1}^\infty \frac{1}{2^j\|f_j\|_k}\left|\langle\theta_1,f_j\rangle-\langle\theta_2,f_j\rangle\right|\]
for two distributions $\theta_1$ and $\theta_2$, and with $\{f_j\}_j\subset C^\infty_c(P)$  a sequence of functions that is dense with respect to the norm
\[\|f\|_k=\sum_{|I|\leq k}\sup_{q\in P}|\partial^If(q)|.\]
We will also need an additional lemma.

\begin{proof}[Proof of Lemma \ref{lem:variationpoint}]
Let $V\subseteq T_pP$ be the subspace that is null for the hessians at $p$ of all the functions in $\posfuncs$:
\[V=\{\textrm{$v\in T_pP:\hessian_p f(v,v)=0$ for all $f\in\posfuncs$}\}.\]
Take coordinates $(x_1,x_2,\dots,x_{\dim P})$ around $p$ such that the vectors
\[\frac{\partial}{\partial x_1},\dots,\frac{\partial}{\partial x_{\dim V}}\in T_pM\]
form a basis of $V$ and $\partial/\partial x_1,\dots,\partial/\partial x_{\dim P}$ is an orthonormal basis of $V$. Assume that $p$ corresponds to the origin in these coordinates. Then $\eta$ must be a linear combination of distributions of the form
\begin{equation*}%\label{eq:normalformdistribution}
\left(\frac{\partial}{\partial x_u}\right)^{e_0}
\left(\frac{\partial}{\partial x_1}\right)^{e_1}
\left(\frac{\partial}{\partial x_2}\right)^{e_2}
\cdots
\left(\frac{\partial}{\partial x_{\dim V}}\right)^{e_{\dim V}}
\delta_p
\end{equation*}
where $e_0\in\{0,1\}$, $u>\dim V$, and the integers $e_1,\dots,e_{\dim V}$ are nonnegative. Condition $\diffcondition$ makes it impossible to have higher derivatives in the directions outside $V$. 

Note that if $\nu_s$ is a family of positive measures such that $\nu_0=\mu$ and 
\begin{equation}\label{eq:smallerdistribution}
 \left.\frac{d\nu_s}{ds}\right|_{s=0} = 
\left(\frac{\partial}{\partial x_1}\right)^{e_1}
\left(\frac{\partial}{\partial x_2}\right)^{e_2}
\cdots
\left(\frac{\partial}{\partial x_{\dim V}}\right)^{e_{\dim V}}
\delta_p,
\end{equation}
and if $\phi$ is the flow of the vector field $\partial/\partial x_u$, then 
\[\left.\frac{d}{ds}\phi_s^*\nu_s\right|_{s=0}=
\left(\frac{\partial}{\partial x_u}\right)^{e_0}
\left(\frac{\partial}{\partial x_1}\right)^{e_1}
\left(\frac{\partial}{\partial x_2}\right)^{e_2}
\cdots
\left(\frac{\partial}{\partial x_{\dim V}}\right)^{e_{\dim V}}
\delta_p.
\]
So we will focus on finding such a family $\nu_s$. In particular, we will assume that $\eta_p$ is of the form given in \eqref{eq:smallerdistribution}. In other words, we will assume that it only involves derivatives in the directions of $V$.

 \begin{lem}\label{lem:infiszero}
For $\eta_p$ as in equation \eqref{eq:smallerdistribution} and for $k=\sum_{i=1}^{\dim V}e_i$, we have
 \[\inf_g\dist_k(g\mu,\eta_p)=0,\]
 where the infimum is taken over all measurable functions $g$ on $P$.
\end{lem}
The reader will find the proof of Lemma \ref{lem:infiszero} below.

Take a strictly-decreasing sequence of positive numbers $\{v_j\}_{j=-\infty}^0$ such that $\sum_j 1/v_j=1$. Let $k$ be as in Lemma \ref{lem:infiszero}. For each $j=0,-1,-2,\dots$, take a measurable function $g_j$ such that $\sup_{q\in P}|g_j|\leq 1$ and 
\[\dist_k(v_jg_j\mu,\eta)<2^j+\inf_{|g|\leq 1}\dist_k(v_jg\mu,\eta).\]
With this definition, Lemma \ref{lem:infiszero} implies that if we let $j\to-\infty$, we get $v_jg_j\mu\to\eta$.

We let, for $\sum_{j=-\infty}^iv_j^{-2}\leq |s|<\sum_{j=-\infty}^{i+1}v_j^{-2},$
\[\nu_s=\left(1+(\sgn s)\left(sv_{i+1}g_{i+1}+\sum_{j=-\infty}^i\frac1{v_j}g_j\right)\right)\mu.\]
By construction, $\nu_s$ is a family of positive measures and its derivative at $s=0$ is $\eta$.

To ensure the measurability of the dependence of this construction in $p$, we further specify the construction as follows. For each $j\in\Z_-$, we take a covering of $P$ by measurable sets $A_j$ of diameter at most $-1/j$. For all $p\in A_i$, we take the same function $g_j$. This ensures that these choices are made in a `measurable' way. The rest of the construction does not depend on arbitrary choices, so the dependence becomes measurable immediately.

The last statement of the lemma follows from the fact that if $\eta_p$ satisfies $\langle\eta,1\rangle=0$, then either $B_h$ satisfies that too, or $e_1=e_2=\dots=e_{\dim P}=0$ and the coordinates can be picked so that the mass is preserved by the flow $\phi_s$ for small-enough $|s|$.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:infiszero}]
 Let $V$ and $x_1,x_2,\dots, x_{\dim P}$ be as in the proof of Lemma \ref{lem:variationpoint}. In a small neighborhood $U$ of $p$ in which the exponential map $\exp_p:T_pP\to P$ is injective, we may define the projection $\proj_V:U\to U\cap\exp_pV$ in the obvious way. 
 
 The distribution $\eta_p$ induces a distribution on $V$, $\bar\eta_p$, defined by
 \[\langle \bar\eta_p, f\rangle = \langle\eta_p,g\cdot(f\circ\exp_p^{-1} \circ \proj_V)\rangle,\quad f\in C^\infty_c(V),\]
 where $g$ is any compactly-supported step-function with $g|_U\equiv 1$. Clearly, if we can find a sequence of functions $g_i:T_pP\to\R$ such that $\dist_k(g_i\exp_{p}^*\mu,\bar\eta_p)$ approaches 0 as $i\to\infty$, then the sequence $\langle (g_i\circ \exp^{-1}_p)\mu,\eta_p\rangle$ will also approach 0 and the lemma will be proved. We may thus assume that $P$ is a Euclidean space $\R^{n}$, that $\mu$ and $\eta_p$ are defined on $\R^{n}$, that $p$ is at the origin of $\R^{n}$, and that the projection $\proj_V$ is linear.
 
 Condition \ref{eq:conditionD} implies that for any open set $A\subseteq U$ that contains $p$, the set $\proj_V(\supp\mu\cap A)$ contains infinitely many vectors, and that these vectors span $V$ as a vector space.
 
 For each $j=1,2,\dots$, let $\{x^j_i\}_{i=1}^\infty\subseteq \supp\mu\subset \R^{n}$ be a sequence of points contained within distance $1/j$ of $p$ and within distance $1/j^2$ of $V$. We also assume that $\{\proj_V x^j_i\}_i$ span all of $V$. For a large-enough finite subset $I_j$ of $\N$, there is always a solution to the problem of finding real numbers $c_{ij}$ such that
 \begin{equation}\label{eq:}
 \langle \eta_p,f\rangle=\lim_{h\to0}\frac{1}{h^k}\sum_{i\in I_j}c_{ij}f(hx^j_i)
 \end{equation}
 for all $f\in C^\infty_c(P)$.
 To see this, note that expanding the right-hand-side as Taylor series in $h$ one obtains a linear system in the variables $c_{ij}$, and that this system has solutions if sufficiently many points $x^j_i$ are available.
 
 For each $j=1,2,\dots$, let $\varepsilon_j>0$ be small enough that the balls $B_{\varepsilon_j}(x^j_i)$ are disjoint. For $q\in B_{\varepsilon_j}(x^j_i)\cap\supp\mu$ for some $i\in I_j$, let
 \[g_j(q) = \frac{c_{ij}}{\mu(B_{\varepsilon_j}(x^j_i))},\]
 and let $g_j(q)=0$ for all other $q\in P$. Then $g_j\mu\to\eta$ as $j\to\infty$ because for each $y\in C^\infty_c(P)$ the set 
 \begin{multline*}
 A(y,R)=\Big\{\sum_{i=1}^N c_iy(x_i):\textrm{$x_i\in B_R(p)\subset P$,  $N\in \N$, and}\\
 \textrm{$\langle\eta_p,f\rangle=\lim_{h\to0}\frac1{h^k}\sum_{i=1}^N c_if(hx_i)$ for all $f\in C^\infty_c(P)$ }
 \Big\}
 \end{multline*}
 contains the value of $\langle g_j\mu,y\rangle$ for $R > 1/j$, and the diameter of $A(y,R)$ tends to 0 as $R\to 0$.
 This proves the lemma.
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:generalfamilies}]
 Assume first that the family $\mu_s$ exists. 
 To prove that Condition \diffcondition\ must hold, let $f\in C^\infty_c(P)$ be a nonnegative function $f\in\posfuncs$, and consider the function
 \[g(s)=\int f\,d\mu_s.\]
 Since $f$ is nonnegative and $\mu_s$ is a positive measure for all $s$, $g$ must be nonnegative as well. Since $g(0)=0$, it must also be true that $g'(0)=0$, and this is equivalent to Condition \diffcondition.
 
 Now assume that we have a measure $\mu$ and a distribution $\eta$ such that Condition \diffcondition\ holds, and let us construct a family $\mu_s$ as in the statement of the theorem. Let $\nu_I$ be the measures as in Lemma \ref{lem:decompositionmeasure}. These induce a measure $\gamma$ on $P$ and a family of distributions $\eta_p$ supported at $p\in P$ such that for all $f\in C^\infty_c(P)$
 \[\eta=\int \eta_p d\gamma(p).\]
 The distributions $\eta_p$ also satisfy Condition \ref{eq:conditionD}.
 From Lemma \ref{lem:variationpoint}, we get families $\mu_s^p$ of measures whose derivatives at 0 are precisely the distributions $\eta_p$. Thus, 
 \[\mu_s=\int\mu_s^pd\gamma(p)\]
 is a family as in the statement of the theorem.
 
 If $\mu$ is a probability, since each $\mu^p_s$ preserves the probability, so does $\mu_s$.
\end{proof}


==> smoothing.tex <==
Denote the exponential map by $\exp_x:T_xM\to M$.

A \emph{mollifier} $\psi\in C_c^\infty(\R)$ is a function such that $\psi(x)=\psi(-x)$, $\int\psi=1$, and $\psi\geq 0$. 

%For a positive number $a>0$ and a mollifier $\psi$, we will use the notation $\psi_a$ for the function $\psi_a(x)=\frac1a\psi(x/a)$. Note that $\psi_a$ is again a mollifier.



Fix a generating tuple of vector fields $F=(F_1,\dots,F_\ell)$. Denote by $\phi^i:M\times \R\to M$ the \emph{flow} of $F_i$:
\[\phi^i_0(x)=0,\quad\frac{d\phi^i_s(x)}{ds}=F_i(\phi^i_s(x)),\quad s\in \R.\]
For fixed $s\in \R$, denote the derivative of the diffeomorphism $\phi^i_s$ by $d\phi_s^i:TM\to TM$. Extend it to a map $d\phi^i_s:T^nM\to T^nM$ by setting
\[d\phi^i_s(x,v_1,v_2,\dots,v_n)=(\phi^i_s(x),d\phi^i_s v_1,\dots,d\phi^i_s v_n).\]

For $f\in \Cinfc$, we will denote by $P_i(f)$ the function given by
\[P_i(f)(x,v_1,v_2,\dots,v_n)=\int_\R f\circ d\phi_s^i(x,v_1,\dots,v_n)\,\psi(s)\,ds.\]
This is a convolution in the horizontal direction $F_i$.
Also, for $f\in \Cinfc$ we let $V(f)$ be the convolution in the vertical direction,
\begin{align*}
 V(f)(x,v_1,\dots,v_n)&=\int_{T_xM}dw_1\psi(|w_1-v_1|)\int_{T_xM}dw_2\psi(|w_2-v_2|)\\
 &\cdots \int_{T_xM} dw_n\psi(|w_n-v_n|)f(x,w_1,w_2,\dots,w_n).
\end{align*}

For $f\in \Cinfc$, we will denote
\[\psi*_Ff=P_1P_2\cdots P_\ell V(f).\]



==> structure.tex <==



%A \emph{smooth differential operator} on $T^nM$ can be written, in local coordinates $(x_1,\dots,x_d,v_{11},\dots,v_{nd})$, as a finite sum
%\[\sum_\alpha f_\alpha\partial^\alpha=\sum_\alpha f_\alpha
%\partial_{x_1}^{\alpha_{x_1}} %\partial_{x_2}^{\alpha_{x_2}}\cdots\partial_{x_d}^{\alpha_{x_d}}
%\partial_{v_{11}}^{\alpha_{v_{11}}}\partial_{v_{12}}^{\alpha_{v_{12}}}\cdots\partial_{v_{nd}}^{\alpha_{v_{nd}}}\]
%where the sum is over all multi-indices with $d(n+1)$ nonnegative entries $\alpha=(\alpha_{x_1},\dots,\alpha_{x_d},\alpha_{v_{11}},\dots,\alpha_{v_{nd}})$. The symbol $\partial_u^j$ stands for the $j$-th partial derivative with respect to the variable $u$.

%Let $F_1,F_2,\dots,F_k$ ($k\geq \dim T^nM=d(n+1)$) be a set of smooth sections of $T(T^nM)$ that generate the entire bundle. 

%Globally, any smooth differential operator can be written in terms of the covariant derivatives $\nabla_{F_j}$ in the directions of the vector fields $F_j$ as a finite sum of the form
%\[\sum_I g_I\partial^I\]
%where $g_I\in\Cinf$ and $I=(i_1, i_2, \dots, i_k)\in \Zplus^k$ are multi-indices with $k$ non-negative integer entries, so that
%\[\partial^I=\nabla_{F_1}^{i_1}\nabla_{F_2}^{i_2}\cdots \nabla_{F_k}^{i_k}\]
%where $\nabla_{F_j}$ stands for the covariant derivative in the direction $F_j$ and $\nabla_{F_j}^m=\nabla_{F_j}\circ\nabla_{F_j}\circ\cdots\circ\nabla_{F_j}$ is the iteration of the covariant derivative $m$ times.

We fix a tuple $F=(F_1,\dots,F_\ell)$ of vector fields on the manifold $P$ that generates all of the tangent bundle $TP$.
As before, we denote by $I$ a multi-index $I=(i_1,\dots,i_\ell)$ with $\ell$ nonnegative entries, and by $\partial^I$ the operator that iteratively takes $i_j$ covariant derivatives in the direction $F_{j}$, $j=1,\dots,\ell$.

\begin{lem}[Structural representation in terms of measures]\label{lem:decompositionmeasure}
A distribution $\eta\in\distributionsP$ can be written as a sum
\begin{equation}\label{eq:decompositionmeasure}
\eta=\sum_I \partial^I\nu_I 
\end{equation}
where $I$ ranges over all multi-indices as above; for each $I$, and $\nu_I$ is a signed measure. For a compact set $K\subseteq P$, 
\[K\cap\supp\nu_I=\varnothing\]
for all but finitely many multi-indices $I$.
\end{lem}

\begin{proof}
Let $k=\dim P$.

Take a partition of unity $\{\xi_j\}_{j\in \N}\subseteq C^\infty_c(P)$ of $P$, that is, a countable set of smooth functions $p_i$ with compact support such that $\sum_j\xi_j(p)=1$ and $\xi_j(p)\geq0$ for all $p\in P$, and $\xi_j(p)=0$ for all but finitely $j\in\N$ at any point $p\in P$. We make the further assumption that the support of each of the functions $\xi_j$ is contained in an open set $U_j\subseteq P$ that is diffeomorphic to a cube $[0,1]^{k}$, and we let $\phi_j:U_j\to [0,1]^{k}$ be the corresponding diffeomorphism. 

We let $\tilde\eta_j$ be the distribution on $[0,1]^{k}$ that results from pushing $\xi_j\eta$ forward to the cube and extending periodically. In other words, for all rapidly-decreasing (Schwartz) functions $f\in C^\infty(\R^{k})$, we let $\tau_zf(x)=f(x-z)$ and
\[
\langle \tilde\eta_j,f\rangle= \sum_{z\in\Z^{k}}\langle \eta,p_j\cdot (\tau_zf)\circ\phi^{-1}_j\rangle.
\]
Like all periodic distributions, $\tilde\eta_j$ is a tempered distribution.
We have
\begin{lem}\label{lem:structuretempered}
 Every tempered distribution is a derivative of finite order of some continuous function of polynomial growth.
\end{lem}

For a proof, see for example {\cite[Theorem 3.8.1]{friedlander}}.

Let $\zeta_j$ be the continuous function of polynomial growth corresponding to $\hat\eta_j$ and let $\alpha_j$ be the multi-index corresponding to the derivative in the lemma, so that
\[\hat\eta_j=\partial^{\alpha_j}\zeta_j.\]
Let $D_j$ be the (smooth) differential operator such that $\phi_j^*\partial^{\alpha_j} = D_j\phi_j^*$, and write
\[\xi_j\eta=D_j\phi^*_j\zeta_j.\]
Since $\zeta_j$ is a continuous function, so is $\phi^*_j\zeta_j$, and hence it induces a measure on $U_j$.
Then we can write
\[\eta=\sum_jp_j\eta=\sum_j D_j\phi_j^*\zeta_j,\]
and since each of the summands on the right can be expressed as a finite sum of derivatives of a continuous function, this proves the lemma.
\end{proof}






